Interacting quantum walks

In this work we present the quantum mechanical computer proposed by Feynman in 1985 and, since then, widely cited but seldom used. The main feature of the model is the presence of a built in clocking mechanism managing for the ordered application of the computational primitives to the input/output register.

==> Brown.tex <==
\section{On the theory of Brownian motion} \label{sec:stochmec}
Let $x(t)$ be a stochastic process (i.e. the position of an electron at time $t$). The trajectory $x(t)$ is, in general, not differentiable. Therefore, to discuss the kinematics of stochastic processes we need a substitute for the derivative.\\
We define the mean \emph{forward} derivative $Dx(t)$ by
\begin{equation}
	Dx(t)=\lim_{\Delta t \rightarrow 0^+} E_t \left(\frac{x(t+\Delta t)-x(t)}{\Delta t}\right),
\end{equation}
where $E_t$ indicates the conditional expectation given the state of the system at time $t$. Thus $Dx(t)$ is again a stochastic process. We define, similarly, the \emph{backward} derivative
\begin{equation}
	D_*x(t)=\lim_{\Delta t \rightarrow 0^+} E_t \left( \frac{x(t)-x(t-\Delta t)}{\Delta t} \right).
\end{equation}
The forward and backward derivatives of the stochastic process $q(t)$ are, in general, different. For example, let's consider the Wiener process $w(t)$ with mean $0$ and covariance $cov(w(t_1),w(t_2))=\sigma^2 min[t_1,t_2]$. It is easy to show that, given the fact that the difference process $(w(t_2)-w(t_1))$ is Gaussian (see also \cite{doob53}, cap VI, for some detail about forward and backward derivatives for a stochastic process). If $x(t)$ is differentiable, then $Dx(t)=D_*x(t)$.\\
Brownian motion plays a central role in the theory of stochastic quantization of Nelson. Since both the theory of Ornstein-Uhlenbeck and that of Eistein-Smoluchowsky convolve in the stochastic description of quantum mechanics, we give a brief account of them in what follows. 
\subsection{Ornstein-Uhlenbeck Brownian motion}
We start by discussing the example of the Ornstein-Uhlenbeck theory of Brownian motion with friction in the presence of a potential $V$. We denote by $\mathbf{x}(t)$, $\mathbf{v}(t)$ the position and the velocity of the Brownian particle at time $t$ respectively, by $m$ its mass and by
\begin{equation}
	\mathbf{K}=-\frac{1}{m} \mathbf{grad}V
\end{equation}
the acceleration of the particle due to the potential $V$.\\
We assume that the system is in thermal equilibrium at temperature $T$ (we should keep in mind this, since things become rather more complicated if the system is out of equilibrium), thus having the Maxwell-Boltzmann distribution. %f(v_x)=\sqrt{\frac{k}{2 \pi}} e^{-k v_x}{2}
Let $m\beta$ be the friction coefficient. Then the Langevin equations are
\begin{equation}\label{eq:langevin}
	\begin{cases}
	d\mathbf{x}(t)= \mathbf{v}(t)dt\\
	d\mathbf{v}(t)=-\beta \mathbf{v}(t) dt+\mathbf{K}(\mathbf{x}(t))+d\mathbf{B}(t);
	\end{cases}
\end{equation}
here $\mathbf{B}(t)$ is a Wiener process representing the residual impacts. The fact that $\mathbf{B}(t)$ is a Wiener process follows immediately from the following physical assumptions: we consider a time-interval $\tau$ small compared to the observation time of the system but of such a magnitude that the movement of the particle at two consecutive time-intervals $\tau$ are to be considered independent \cite{einstein56}. This two hypothesis translate in the following:
\begin{theorem}
Let $p^t$, $0\leq t < \infty$, be a family of probability measures on $\mathbb{R}$ such that:
\begin{enumerate}
\def \theenumi{\roman{enumi}}
\item $ p^t * p^s = p^{t+s}$, with $ 0 \leq t,s < \infty$, where $*$ denotes the convolution;
\item $\lim_{t \to 0}{p^t ( \{ x: |x| \geq \epsilon \})}$ = o(t);
\item for $ t \geq 0$, $p^t$ is invariant under transformation $x \rightarrow -x$.
\end{enumerate}
Then either $p^t = \delta, \forall t \geq 0$ or there is a $D > 0$, such that, for all $t > 0$, $p^t$ has the density
\begin{equation}
	p(t,x) = \frac{1}{\sqrt{4 \pi D t}} \; e^{-\frac{x^2}{4 D t}}
\end{equation}
so that $p$ satisfies the diffusion equation
\begin{align}
	& &\frac{\partial p}{ \partial t} =   D \frac{\partial ^2 p}{\partial ^ 2 x}  & &  t >0.
\end{align}
\end{theorem}
For the proof of the theorem we refer the  reader to \cite{nelson67} (\S 5 pp. 23-31).\\
Since the difference of Wiener processes $w(t)-w(s), 0 \leq s \leq t <\infty$  form a Gaussian process of mean $0$ and variance
\[
E[(w(t)-w(s))(w(t')-w(s'))]= \sigma^2|[s,t] \cap [s',t']|
\]
the $d\mathbf{B}(t)$ are Gaussian with mean $0$ and variance determined by the diffusion constant of the medium; in this case we have  
\begin{equation}
	E d\mathbf{B}(t)^2=\frac{6 \beta k T}{m} dt,
\end{equation}
where $E$ denotes the expectation with respect to the Gaussian measure and $k$ is the Boltzmann constant.\\
Without loss of generality we can give an example in the one dimensional case of a particle moving on a line. If $v(0)=v_0$ and $x(0)=x_0$ the solution of the initial value problem is,
\begin{eqnarray}
v(t)& = & e^{-\beta t} v_0 + e^{-\beta t} \int_0 ^ t e^{\beta s} dB(s) \label{eq:vmedia}\\
x(t)& = & x_0 + \int_0 ^ t v(s) ds.
\end{eqnarray}
The random variables $v(t)$ are Gaussian with mean
\[
\bar{v}(t)=e^{-\beta t} v_0,
\]
and covariance
\[
r(t,s)= \frac{D}{\beta} \left (  e^{-\beta|t-s|} -e^{-\beta(t+s)} \right ).
 \]
The Gaussian measure $\mu$ with mean $0$ and variance $\beta D$ is invariant, $P^{t^*} \mu = \mu$, and $\mu$ is the limiting distribution of $v(t)$ as $t \to \infty$.\\
We observe that the $d\mathbf{B}(t)$ are independent of the $\mathbf{x}(s),\mathbf{v}(s)$ for $s \leq t$. Then there is an asymmetry in time: we may also write the Langevin equations \eqref{eq:langevin} as
\begin{equation} \label{eq:langevinback}
	\begin{cases}
	d\mathbf{x}(t)= \mathbf{v}(t)dt\\
	d\mathbf{v}(t)=\beta \mathbf{v}(t) dt+\mathbf{K}(\mathbf{x}(t))+d\mathbf{B_*}(t);
	\end{cases}
\end{equation}
where the $d\mathbf{B_*}(t)$ are independent of $\mathbf{x}(s),\mathbf{v}(s)$ for $s \geq t$. We observe that this form of the Langevin equations takes into account the backward evolution of the system, thus the change in the sign of the friction coefficient; the acceleration $\mathbf{K}$ has the same sign because it is not dependent of time.\\
It is known that in the Ornstein-Uhlenbeck theory of Brownian motion the trajectories $\mathbf{x}(t)$ are differentiable, that is
\begin{equation}
	D\mathbf{x}(t)=D_*\mathbf{x}(t)=\frac{d\mathbf{x}(t)}{dt}=\mathbf{v}(t)
\end{equation}
On the other side, since $d\mathbf{B}(t)$ is of order $dt^{1/2}$, $\mathbf{B}(t)$, and then $\mathbf{v}(t)$, is not differentiable. We can nevertheless apply the \emph{substitute} of the derivative operator to $\mathbf{v}(t)$; since $\mathbf{B}(t+\Delta t)-\mathbf{B}(t)$, with $\Delta t >0$, is independent of the history of the process and has expectation $0$, we obtain  $D\mathbf{B}(t)=0$ and, remembering that $D$ is a linear operator, we have
\begin{equation} \label{eq:velocityforw}
	D\mathbf{v}(t)=-\beta \mathbf{v}(t)+ \mathbf{K}(\mathbf{x}(t))
\end{equation}
and
\begin{equation}\label{eq:velocityback}
	D_*\mathbf{v}(t)=\beta \mathbf{v}(t)+ \mathbf{K}(\mathbf{x}(t)).
\end{equation}
If $\mathbf{K}=0$ (free particle), we see that $D\mathbf{v}(t)=-D_*\mathbf{v}(t)=-\beta \mathbf{v}(t)$, which reflects the dumping effect of friction, resulting in a general trend of the velocity toward $0$, independently of the choice of the direction of time.\\
It follows from \eqref{eq:velocityforw} and \eqref{eq:velocityback} that
\begin{equation}
	\frac{1}{2}DD_* \mathbf{x}(t)+\frac{1}{2}D_*D \mathbf{x}(t) = \mathbf{K}(\mathbf x(t))
\end{equation}
Remembering the Newton's law $\mathbf{F}=m\mathbf{a}$, we define the \emph{mean second derivative} or \emph{acceleration} of a stochastic process to be
\begin{equation}\label{eq:meanacceleration}
	\mathbf{a}(t)=\frac{1}{2}DD_* \mathbf{x}(t)+\frac{1}{2}D_*D \mathbf{x}(t) = \mathbf{K}(\mathbf x(t));
\end{equation}
using an analogy to classical kinematics, we define $D$ and $D_*$ to be, respectively, the \emph{forward} and \emph{backward} velocity.\\
The O-U theory of Brownian motion allows for the description of the system in the phase-space; furthermore, Newtonian dynamics can be brought into the stochastic theory by means of a mean derivative concept which, in turn, bypasses the difficulty due to the time-asimmetry typical of the diffusion processes.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Einstein-Smoluchowsky Brownian motion}
The Einstein-Smoluchowsky (E-S) theory for the Brownian motion is an approximation of the Ornstein-Uhlenbeck (O-U) under two hypothesis:
\begin{itemize}
\item the friction coefficient $\beta$ is large;
\item we consider the process on a time scale larger than the relaxation time $\beta^{-1}$.
\end{itemize}
\begin{figure}[ht]
	\includegraphics{figrel.eps}
	\caption{The figure represents the average velocity of the diffusion process for different values of the \emph{friction} parameter $\beta$: the arrow indicates the decreasing direction of $\beta$.}
	\label{fig:relaxation}
\end{figure}
The first hypothesis implies that external forces $\mathbf{F}$ do not accelerate the particle but simply imparts a velocity $\mathbf{F}/m \beta$ to the particle; the second one make it possible to characterize statistically the motion of the free Brownian particle as a Wiener process $\vec{\eta}(t)=\{\eta_1(t),\eta_2(t),\eta_3(t)\}$ with
\begin{eqnarray}
	Ed\vec{\eta}(t)&=&0 \label{eq:meaneta} \\
	Ed\eta_i(t)\eta_j(t')&=&2 \alpha \delta_{ij}\delta(t-t') \label{eq:correta}.
\end{eqnarray}
where $\alpha$ is a diffusion constant defined as
\begin{equation}
	\alpha=\frac{k_B T}{m \beta},
\end{equation}
$m$ being the mass of the particle.\\
An example of how the E-S theory can be derived by the O-U one via a time-scale transformation can be found in \cite{namiki92}.\\
Considering the case in which there are external forces (or currents) acting on the particle, the position $\vec{x}(t)$ of the Brownian particle satisfies
\begin{equation} \label{eq:fito}
	d\vec{x}(t)=\vec{b}(\vec{x}(t);t)dt+d\vec{\eta}(t)
\end{equation}
$\vec{\eta}$ being the Wiener process of above and $\vec{b}$ a vector-valued function on space-time.\\
Since the $d\vec{\eta}(t)$ are independent of the past, the mean forward velocity is
\begin{equation}
	D\vec{x}(t)=\vec{b}(\vec{x}(t);t).
\end{equation}
For the sake of time symmetry we write the differential equation associated to the process as
\begin{equation}
		d\vec{x}(t)=\vec{b}_*(\vec{x}(t);t)dt+d\vec{\eta}_*(t),
\end{equation}
where the $d\vec{\eta}_*(t)$ have the same properties of $d\vec{\eta}_(t)$ but are independent of the future; it follows immediately that the \emph{mean backward velocity} is
\begin{equation}
	D_*\vec{x}(t)=\vec{b}_*(\vec{x}(t);t).
\end{equation}
Let $\rho(\vec{x};t)$ be the probability density of $\vec{x}(t)$; then $\rho$ satisfies the \emph{forward Fokker-Planck} equation
\begin{equation}\label{eq:ffp}
	\frac{\partial \rho}{\partial t}= -div(\vec{b}\rho)+ \alpha \Delta \rho,
\end{equation}
with $\Delta = \nabla ^2$, and the \emph{backward Fokker-Planck} equation
\begin{equation}\label{eq:bfp}
	\frac{\partial \rho}{\partial t}= -div(\vec{b}_*\rho)-\alpha \Delta \rho.
\end{equation}
The average of \eqref{eq:ffp} and \eqref{eq:bfp} yields to the continuity equation
\begin{equation}
		\frac{\partial \rho}{\partial t}= -div(\vec{v}\rho),
\end{equation}
where
\begin{equation}
	\vec{v}=\frac{1}{2}( \vec{b}+ \vec{b_*}).
\end{equation}
We call $\vec{v}$ the \emph{current velocity}.\\
Given a function $f$ of $\vec{x}$ and $t$, to calculate $Df(\vec{x}(t);t)$ we take the Taylor expansion up to the first order in $t$ and to the second order in $d\vec{x}$
\begin{eqnarray}
	d f(\vec{x}(t);t) & = & \frac{\partial f}{\partial t}(\vec{x}(t);t)+ d \vec{x}(t)\cdot \nabla f(\vec{x}(t);t)+ \nonumber \\ 
	& & +\frac{1}{2} \sum_{i,j}dx_i(t) dx_j(t) \frac{\partial ^2 f}{\partial x_i \partial x_j} (\vec{x}(t);t);
\end{eqnarray}
this choice takes into account the non-differentiability of the diffusion part of the process $d\vec{x}(t)$ with respect to time.
From \eqref{eq:fito} follows that we can replace the $dx_i$ with the $d\eta_i$ and, when we take the expectation conditional on $\mathcal{P}_t$, or the past of the process, we have that $d \vec{x}(t)\cdot \nabla f(\vec{x}(t);t) = d \vec{b}(\vec{x}(t);(t))\cdot \nabla f(\vec{x}(t);t)$ since $\vec{\eta}(t)$ is independent of $\vec{x}(t)$ and has mean $0$.\\
Then, remembering the definition \eqref{eq:correta}, we obtain
\begin{equation}
	Df(\vec{x}(t);t)=  \left( \frac{\partial}{\partial t} + \vec{b}\cdot \nabla + \alpha \Delta \right )f(\vec{x}(t);t)
\end{equation}
and, for the backward evolution,
\begin{equation}
	D_*f(\vec{x}(t);t)= \left ( \frac{\partial}{\partial t} + \vec{b_*}\cdot \nabla - \alpha \Delta \right) f(\vec{x}(t);t).
\end{equation}
Using the invariance on space-time of the distribution $\rho d^3x dt$ (remember that the system is at thermal equilibrium) and the Fokker-Planck equation (we refer to \cite{nelson67} and \cite{nelson85} for an exhausive explanation), we obtain
\begin{equation}
	\vec{b}_*=\vec{b}-2 \alpha (\Delta \rho)/\rho
\end{equation}
or
\begin{equation}
	\vec{u}=  \alpha (\Delta \rho)/\rho
\end{equation}
where
\begin{equation}
	\vec{u}= \frac{1}{2} (\vec{b}-\vec{b}_*).
\end{equation}
According with Einstein theory, $\vec{u}$ is the velocity acquired by a Brownian particle, in equilibrium with an external force, to balance the osmotic pressure forces of the suspension: $\vec{u}$ is in fact usually referred as the \emph{osmotic velocity}.

==> Guerrapresc.tex <==
\subsection{The prescription of Guerra.}
We begin with the state of a simple system consisting of $2s+1$ spin $1/2$ particles $\sigma(i)=(\sigma_1(i),\sigma_2(i),\sigma_3(i))=(\sigma_x(i),\sigma_y(i),\sigma_z(i))$ on a linear regular lattice with distance $\epsilon$; the indexes $x,y,z$ indicate the axis of a given reference frame.
We choose the basis of the simultaneous eigenvalues of the $\sigma_z(i)$ operators. The basis vectors are then of the form
\[
| \sigma_z(-s)=\pm 1, \sigma_z(-s+1)=\pm 1, \ldots, \sigma_z(s)=\pm 1 \rangle,\]
or, 
\[
\underbrace{| \pm 1, \pm 1, \ldots, \pm 1 \rangle}_{2s+1}.
\]
%We will refer to this basis as \emph{computational basis}.\\
The system evolves under the Hamiltonian
\begin{equation}
	H_s=\sum_{i=1}^{s-1}\lambda (\sigma_+(i+1)\sigma_-(i)+ \sigma_+(s-(i+1))\sigma_-(s-i)+ Hermitian \; conjugate), 
\end{equation}
where $\lambda$ is a constant.\\
In our setup, the initial state of the system is the eigenstate corresponding to the eigenvalue $n=1$ of the operator
\begin{equation}
	N=\sum_{i=-s}^s \frac{1+\sigma_z(i)}{2},
\end{equation}
which does nothing more than to count the number of spin up in the chain. Since $[H,N]=0$ the number of spin up, or \emph{excitations}, in the chain is a constant of motion. The operator
\begin{equation}
	Q=\sum_{i=-s}^s i \; \frac{1+\sigma_z(i)}{2}
\end{equation}
is then well defined and indicates the position of the excitation. Thus the space in which the system evolves is a proper subspace of the Hilbert space $\mathcal{H} \approx (\mathbb{C}^2)^{2s+1}$. A suitable basis for the space spanned by the evolution of the system is the one in which $Q$ is diagonal. We will indicate the $i$-th vector of the basis as
\[
\ket{Q=i}=\ket{-1,\ldots,\stackrel{i-1}{-1},\stackrel{i}{1},\stackrel{i+1}{-1},\ldots,-1}
\]
The Schr\"odingrer equation is then
\begin{equation}
	i \hbar \partial_t \psi = - \frac{\hbar}{2m} H \psi
\end{equation}
where $\psi$ is a function from $\mathbb{Z}\cap [-s,s] \times \mathbb{R}$ into $\mathbb{C}$.\\
The matrix form of the H operator is
\[
 \lambda \left(
\begin{array}[5]{c c c c c c}
	0 & 1 & 0 &\ldots & 0 & 0 \\
	1 & 0 & 1 &\ldots & 0 & 0 \\
	0 & 1 & 0 &\ldots & 0 & 0 \\
	\ldots & \ldots & \ldots &\ldots & \ldots &\ldots \\
	0 & \ldots & \ldots &\ldots & 0 & 1\\
	0 & \ldots & \ldots &\ldots & 1 & 0\\
\end{array} 
\right)
\]
which, if we assign $\lambda = -\hbar/2m \epsilon ^2$ is the finite difference approximation of the Laplacean $\nabla ^2$ (the diagonal terms  can be restored by a shift in the energy). Since we are not studying the limiting behavior of the system as $\epsilon \rightarrow 0$ we can set, without loss of generality, $\lambda = -1$.\\
In order to avoid reflection on the boundaries, we are going to extend the system letting $s \rightarrow \infty$. Given the  initial condition $\psi(j,0)=\psi_j(0)=\delta_{j,k}$ the solution of the Sch\"odinger equation is
\begin{equation}
	\psi_j(t)= i^{j-k} J_{j-k}(t)
\end{equation}
where $J_k(t)$ is a Bessel function of the first kind.\\
Obviously the operator $H$ can no longer be defined as a matrix; we give then the \emph{implicit} definition of the Hamiltonian, in the position basis:
\begin{equation}
\begin{cases}
 H_{n \; n'}=1 & if  |n-n'|=1 \\
 0 & otherwise
\end{cases} 
\end{equation}
With this notations, the continuity equations become
\begin{eqnarray}
	\dot{\rho}_n & = & \sum_{n'} a_{nn'} \rho_{n'} \\
	a_{nn'} & = & \left ( \frac{\rho_{n'}}{\rho_n}\right ) ^{1/2} \sin({S_{n'}-S_n})  
\end{eqnarray}
where the sum is restricted to $|n-n'|=1$.\\
We observe that, given the lattice constant $\epsilon$, $\frac{S_{n'}-S_n}{\epsilon}$  is the lattice approximation of the gradient. Thus we define a vector field on the lattice, defined as
\begin{equation}
	v(n',n)= 2 \epsilon a_{n'n} \left( \frac{\rho_n}{\rho_{n'}}\right )^{1/2}
\end{equation}
Starting from this definition, Guerra shows that the discrete continuity equations reproduce correctly the continuous one \cite{guerra84}, \cite{guerra88}.\\
The forward derivative summarizes all random properties of the system. It can be easily shown that, given the lattice approximation we defined above, we can write
\begin{equation} \label{eq:forwtrans}
	a_{n'n}^+ =  \left ( \frac{\rho_{n'}}{\rho_n}\right ) ^{1/2} \left( 1+\sin({S_{n'}-S_n}) \right).
\end{equation}
Thus, if we define the  coefficients $a_{n'n}^+$ for each time $t$, we can generate the Markov process associated to the system... and it is exactly what we are going to do in the next section!
 
%NOTA: potenziale di Bohm pressione osmotica generata dalla densità di probabilità dello spazio campionario\\


==> Madelung.tex <==
\subsection{Madelung fluid and Markov processes}
In 1984 Guerra and Marra gave a definition of the \emph{discrete} stochastic variational principle which can be seen as an approximation of the continuous case (to which it reduces in the limiting case thus proving the correctness of the approximation)\cite{guerra84}.\\
In a quantum system living in a \emph{separable} Hilbert space Guerra associates a Markov process. In this section we are going to see the general ``receipt'' to do it.\\
We consider a quantum system living in a separable Hilbert space and choose the basis $\phi_i, \; i=1,2,\ldots$. Any function $\psi$ has then the decomposition $\psi_i= \braket{\phi_i}{\psi}$. The Schr\"odinger equation has the following form
\begin{equation} \label{eq:schrosep}
	i \hbar \dot{\psi}_i = \sum_j h_{i,j} \exp(i\; \alpha_{i,j}) \psi_j.
\end{equation}
Since the Hamiltonian is an Hermitian operator, it follows that $h_{i,j} = h_{j,i}$ and $\alpha_{i,j}=-\alpha_{j,i}, \; \alpha_{i,i}=0$. It is convenient to change the variables using the Madelung transform so that
\[
\psi_i=\rho_i^{1/2} \exp(i S_i / \hbar).
\]
Then \eref{eq:schrosep} is split into two real equations, one for the densities $\rho_i$ and the other for the phase velocities:
\begin{eqnarray} 
	\dot{\rho}_i = \sum_j (\frac{2 h_{i,j}}{\hbar})(\rho_i\rho_j)^{1/2} \sin{\beta_{i,j}} \label{eq:cont}\\
	\dot{S}_i = - \sum_j (\frac{2 h_{i,j}}{\hbar})(\frac{\rho_i}{\rho_j})^{1/2} \cos{\beta_{i,j}} \label{eq:HJ}
\end{eqnarray}
where
\begin{equation}
	\beta_{i,j}=\frac{\alpha_{i,j}+S_j+S_i}{\hbar},\; \beta_{i,j}= -\beta_{j,i},\;\beta_{i,i}=0.
\end{equation}
Since \eqref{eq:cont} is a continuity equation
\begin{equation}
	\sum_i \rho_i(t)=1
\end{equation}
if it was at $t=0$.\\
The functions \eqref{eq:cont} and \eqref{eq:HJ} have other interesting properties which describe the quantum features of the physical system \cite{guerra84}.\\
A stochastic process is a Markov process if its time-evolution \emph{depends only of the actual state of the system}. Consider a Markov process $q(t)$ taking values on the set ${1,2,\ldots}$. Let $\rho_i(t)$ be the occupation probability of the state $i$ at time $t$; given a function $F$ of $q(t)$ and $t$ its expectation is
\begin{equation}
	E(F(q(t),t))=\sum_i F_i(t) \rho_i(t).
\end{equation}
We introduce the transition probabilities $p(t,i;t',j)$ (read it as: probability of being in the state $i$ at time $t$ given that we were in the state $j$ at time $t'$), $t \geq t'$, which satisfy the following properties:
\begin{itemize}
\item \[ p \geq0, \sum_i p(t,i;t',j)=1; \]
\item \[ \lim_{t \to t^{'+}} p(t,i;t',j) =\delta_{ij}; \]
\item \[ p(t,i;t',j) = \sum_k p(t,i;t'',k)p(t,i;t',j),\; t \geq t'' \geq t'\; \mbox{(chain rule)}; \]
\item \[\rho_i(t)=\sum_j p(t,i;t',j) \rho_j(t).\]
\end{itemize}
Assume the existence of the limit
\begin{equation}
	a_{ij}^+(t)= \lim_{\Delta t \to 0^+} \frac{p(t+\Delta t,i;t,j) -\delta_{ij}}{\Delta t}.
\end{equation}
Then we have:

\begin{eqnarray}
a_{ij}^+ \geq 0 \mbox{ for } i \neq j&, & \nonumber \\ 
\sum_i a_{ij}^+(t)=0 &; & \nonumber \\ 
a_{ii}^+ =0&, & \nonumber
\end{eqnarray}
and the forward diffusion equation
\begin{eqnarray}
\partial_t p(t,i;t',j)& = & \sum_i a_{ik}^+ (t) p(t,k;t',j) \\
\dot{\rho}_i(t) & = &  \sum_j a_{ij}^+ (t) \rho_j(t) \label{eq:master}
\end{eqnarray}
Equation \eqref{eq:master} is sometime referred as \emph{master equation}.

==> Nelsquant.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Nelson's stochastic quantization}
In the previous section we introduced the O-U and E-S theories of Brownian motion; as already said, the second one applies when the friction coefficient is large and on a more coarse-grained time scale.\\
The \emph{universal Brownian motion hypothesis} affirms that particles in empty space, or \emph{ether}, undergo a Brownian motion. Since macroscopic bodies do not exhibit such a behavior, Nelson assumes that the diffusion coefficient $\alpha$ is inversely proportional to the mass of the particle, let's say
\begin{equation}
	\alpha= \frac{\hbar}{2m} 
\end{equation}
where $\hbar$, for the time being, is just a constant which has the dimension of an action.\\
Since we are in the ether, Brownian motion will be not smooth and velocity can not exist; therefore, we can not describe the state of a particle as a point in the phase-space. On the other side, since there is no friction, we are out of the application range of the E-S theory. We can nevertheless try to describe the motion of the particle as a Markov process, thus actually using the E-S theory.\\
Putting ourself in this context rises another problem: in the E-S theory the action of an external force  $\vec{F}$ on a particle impresses to the latter a velocity $F/m\beta$ because of the \emph{damping} effect of the friction. In the theory of Nelson the dynamic will be given by Newton's law $F=ma$. Thus it becomes necessary a fusion of the two theories of Brownian motion: the kinematics will be that of E-S while the dynamics will be that of O-U.\\
In what follows we give a brief account of the prescription of Nelson to associate to the evolution of a quantum system a stochastic process\cite{nelson85}.\\

 
The state of an isolated quantum system with $n$ degrees of freedom is given by a complex valued function on $\mathbb{R}^n \times \mathbb{R}$, say $\psi(x_1,x_2,\ldots,x_n ; t)=\psi(\vec{x};t)$, which is the solution of the Schr\"odinger equation
\begin{equation}
\begin{cases}
i\hbar \frac{\partial \psi}{\partial t}  = -\sum_{i=1}^n \frac{1}{2 m_i}\frac{\partial ^2 \psi}{\partial x_i^2}+V(t)\psi = -\frac{1}{2}\nabla^2 \psi + V(t)\psi \\
\psi(0)=\psi_0,
\end{cases}
\end{equation}
where $\psi(0)$ indicates the state of the system at $t=0$ and $V(x_1,x_2,\ldots,x_n;t)=V(\vec{x};t)$ is a real valued function representing the potential energy. By taking all the masses equal to one and $\hbar=1$, the Schr\"odinger equation assumes the simpler form
\begin{equation} \label{eq:schro}
	i \frac{\partial \psi}{\partial t} = -\frac{1}{2}\nabla^2 \psi + V(t)\psi
\end{equation}
%where $\psi = \psi(x_1,x_2,\ldots,x_n ; t)$ is a complex valued function on $\mathbb{R}^n \times \mathbb{R}$ and $V(t)$ is the operation of multiplication by the real valued function $V(x_1,x_2,\ldots,x_n;t)$, which represents the potential energy. 
In quantum mechanics $|\psi(\vec{x};t)|^2$ represents the probability density of the result of measuring the position of the system at time $t$. This interpretation makes sense only if, $\forall t \in \mathbb{R}$,
\begin{equation} \label{eq:unity}
\int_{\mathbb{R}^n}|\psi(x;t)|^2 dx =1.
\end{equation}
It is known that, under suitable restriction for the potential $V(t)$, the equation \eqref{eq:schro} has an unique solution and the integral \eqref{eq:unity} is independent of time.\\
For the sake of simplicity, we are going to associate a stochastic process to the trajectory of a single free particle, say an electron, moving on a line; the state of the electron is the function $\psi:\mathbb{R}\times \mathbb{R}\rightarrow \mathbb{C}$, which is a solution of \eqref{eq:schro}.\\
To construct the corresponding stochastic theory, let us write, following the prescription of Nelson \cite{nelson66} 
\[
\psi(x;t)=\exp{(R(x;t)+i S(x;t))}.
\]
From the probabilistic interpretation of $|\psi(x;t)|^2$, it follows immediately that, given the initial condition $\rho(x;0)=|\psi(x;0)|^2$, the stochastic process ``trajectory of the electron'' at time $t$ has the probability density
\begin{equation}\label{eq:density}
\rho(x;t)=|\psi(x;t)|^2=\exp(2 R(x;t)).
\end{equation}
If we define
\begin{equation} \label{eq:forward2}
	b(x;t)=\nabla R(x;t)+\nabla S(x;t)
\end{equation}
the solution of the stochastic differential equation of Ito's type
\begin{equation} \label{eq:stochdiff}
	dx(t)=b(x(t);t)dt+dw(t)
\end{equation}
with initial probability density $\rho(x;0)=|\psi(x;0)|^2$, is exactly \eqref{eq:density}\footnote{The term $w(t)$ is a Wiener process in one dimension, normalized so that the variance $w(s_2)-w(s_1)$ is $|s_2-s_1|$; the probability density of $w(s_2)-w(s_1)$ is $2 \pi |s_2 - s_1|^{-\frac{1}{2}} \exp{(-x^2)/2 |s_2-s_1|}$.}.\\
It is worth noticing that the choice of $b$ is arbitrary, and that the arbitrariness of the process which leads from the Schr\"odinger equation to the associated stochastic process stay therein.\\
%%It is worth noticing that the function $b(x(t);t)$ usually indicates the mean forward velocity, defined in \cite{nelson66} as
%%\begin{equation} \label{eq:forward1}
%%Dx(t)=	\lim_{\Delta t \rightarrow 0^+} E \left [ \frac{x(t+\Delta t)-x(t)}{\Delta t} \right ];
%%\end{equation}
%for the time being let us assume that the definitions \eqref{eq:forward1} and \eqref{eq:forward2} are equivalent.\\
What \eqref{eq:density} says is that $\rho$ satisfies
\begin{equation}\label{eq:probdiff}
	\frac{\partial \rho}{\partial t} = -div (b\rho)+\frac{1}{2}\nabla^2(\rho). 
\end{equation}
The term $b(x(t);t)dt$ in \eqref{eq:stochdiff} corresponds to the term $-div (b^+\rho)$ in \eqref{eq:probdiff} and the Wiener process in \eqref{eq:stochdiff} corresponds to the Laplacean in \eqref{eq:probdiff}.\\
Thus in stochastic mechanics the motion of the quantum mechanical system is governed not by the Schr\"odinger equation \eqref{eq:schro} but by a stochastic differential equation \eqref{eq:stochdiff}.

==> ccnot.tex <==
\section{The C-C-NOT gate} \label{sec:ccnot}
By setting the operator $A=\sigma_1(c)$ and $B=1$ we implement the  CONDITIONAL NOT$(\rho,c)$, or C-NOT$(\rho,c)$, gate. The C-NOT is a logical \emph{reversible} binary operator whose truth table is given in table \ref{tab:truthCNOT}\footnote{The C-NOT can also be seen as a \emph{reversible} version of the binary sum.}.
\begin{table*}[h]
	\centering
		\begin{tabular}{||c | c || c | c||} \hline
			$\rho$ & $c$ &$\rho'$ & c' \\ \hline \hline
			0 & 0 &0 & 0  \\ \hline
			0 & 1 &0 & 1  \\ \hline
			1 & 0 &1 & 1  \\ \hline
			1 & 1 &1 & 0  \\ \hline\hline
		\end{tabular}
	\caption{The truth table of the C-NOT; $\rho$ and $c$ are the input values whereas $\rho'$ and $c'$ are the output values.}
	\label{tab:truthCNOT}
\end{table*}\\
With the choice $A=SWITCH(\rho(2),\sigma_1(c),I)$ and $B = I$, where $\rho(1)$ and $\rho(2)$ are controlling qubits, we realize the circuit
\begin{equation}
	SWITCH(\rho(1),SWITCH(\rho(2),\sigma_1(c),I),I)
\end{equation}
also known as \emph{CONTROLLED-CONTROLLED-NOT}, or \emph{CCNOT}. This logical reversible operator forms a \emph{complete logical basis for the set of reversible boolean functions}. The action on the computational basis is reported in table \ref{tab:truthCCNOT}.
\begin{table*}[h]
	\centering
		\begin{tabular}{||c | c | c || c | c| c||} \hline
			$\rho(1)$ & $\rho(2)$ & $c$ & $\rho(1)'$ & $\rho(2)'$ & c' \\ \hline \hline
			0 & 0 & 0 & 0 & 0 & 0  \\ \hline
			0 & 0 & 1 & 0 & 0 & 1  \\ \hline
			0 & 1 & 0 & 0 & 1 & 0  \\ \hline
			0 & 1 & 1 & 0 & 1 & 1  \\ \hline
			1 & 0 & 0 & 1 & 0 & 0  \\ \hline
			1 & 0 & 1 & 1 & 0 & 1  \\ \hline
			1 & 1 & 0 & 1 & 1 & 1  \\ \hline
			1 & 1 & 1 & 1 & 1 & 0  \\ \hline \hline
		\end{tabular}
	\caption{The truth table of the C-NOT; $\rho$ and $c$ are the input values whereas $\rho'$ and $c'$ are the output values.}
	\label{tab:truthCCNOT}
\end{table*}\\
The possibility of implementing the \emph{CCNOT} gate makes the Feynman quantum computer \emph{universal} with respect to the computation of boolean function. In other words the class of function computable by a Feynman machine is at least as big as the class of partial recursive functions. 
\begin{figure}[h]
	\centering
		\includegraphics[width=10cm]{Figure/CCNot.eps}
	\caption{The circuit implementing the CCNOT gate.}
	\label{fig:CCNot}
\end{figure}\\
(SERVE DIRE CHE PER SET UNIVERSALE DI GATE PER CALCOLATORE QUANTISTICO REVERSIBILE SERVE ANCHE IL PHASE SHIFT)....


==> chap_introduction.tex <==
\chapter{Introduction}
%
\section{Physics and computation}
The intimate notion of \emph{computability}  depends on the possibility of implementing the physical process transforming a given \emph{input state} in the desired \emph{output state}. This was already clear to von Neumann \cite{vonNeumann76} which, in the late Seventies, suggested a renewal of the communication between physics and computer science. The Church-Turing hypothesis \cite{church36,turing36,kleene43} 
\begin{quotation}
Every 'function that would naturally be regarded as computable' can be computed by a universal Turing machine
\end{quotation}
itself, in fact, makes an implicit physical assertion:  the idea of computable function is related to the possibility of physically implement the process (algorithm) computing it.  This kind of unified approach to  physics and information science goes under the name of \emph{information mechanics} \cite{toffoli82} \footnote{Toffoli illustrated the equivalence between a physical experiment and a computing process by means of the following example:
\begin{quote}
Let us suppose that intelligent beings are observing us from a far away star. How could them understand whether we are carrying on a computation or a physical experiment? They could not understand it from what we are doing since there is no objective difference. The difference is in our intentions, in our knowledge, in our expectations.
\end{quote}}.\\
On the other side, computers may help in the simulation of physical systems; the question is: up to which complexity? The idea to use a quantum mechanical universal computer to simulate quantum mechanical systems may be traced back to Feynman \cite{feyn82};he showed, in fact, that the simulation of the evolution of a quantum system on a classical computer requires an  amount of resources which scales exponentially with the dimension of the system, that is, it is an \emph{intractable problem}. Feynman argued that quantum mechanical systems are well equipped to simulate other quantum mechanical systems;  hence a universal quantum machine might be able to \emph{efficiently} do such simulations.\\
The proof that a quantum universal computer would be exponentially more efficient than any classical one in the simulation of quantum mechanical systems suggests to use quantum computing device to address other computational tasks, with the hope of getting the same exponential speed-up.\\ [5pt]
(Nowadays quantum computer science has become a mature interdisciplinary research field: any field of classical information science has an analogous in quantum information science: algorithmics (cita deutsch, jozsa, grover, shor, simon, kempe, e articoli di review), information theory (schumacher, e riferimenti in datta), cryptography (bennett brassard), communication, correcting codes; on the other side, the need of a physical support for quantum computation has motivated a huge amount of research in optics, condensed matter physics, spintronics and so on (QUALCHE ARTICOLO DI RIFERIMENTO, MEGLIO SE RECENTE). Although very far away from a commercial version of a quantum computer, there are already companies selling cryptographic devices implementing quantum communication protocols (BB84) via optic fibers.\\[5pt]
In our intentions, this introductory chapter would be a guide through the literature needed to get the main ideas about methods and concepts of quantum computation.)
%
%
%
\section{The Church-Turing-Deutsch principle and  quantum complexity theory}
%
In 1985 David Deutsch \cite{deutsch85} tried to explicit the implicit physical assertion of the Church-Turing hypotheses expressing stating it as follows:
\begin{quote}
Every finitely realizable physical system can be perfectly simulated by a universal model computing machine operating by finite means.
\end{quote}
This modified version of the Church-Turing hypothesis is known as the \emph{Church-Turing-Deutsch principle} and we refer to the paper of Deutsch for a full explanation of it; there are anyway a couple of points it is worth highlighting: first of all, this principle is stronger than the original one; at first sight, it seems that there are processes, such as the ones associated to any continuum system, which cannot be perfectly simulated by finite means. But if our universal computing device is able to simulate, by finite means, any finitely realizable quantum system, then it is able to simulate any real physical system (after all the world is quantum mechanical). Secondly, by finite means it is intended a machine that in each quantum of time operates only on a finite subsystem of the overall system and  depending on a finite subsystem and following rules that can be finitely mathematically defined (for example by integers).\\
Quantum Turing machines are not able to compute non-recursive functions.\\
Factoring is not NP-Complete\\
BPP is not BQP\\
The role played by the quantum Turing machine in quantum complexity theory is analogous to the one played in classical complexity theory by the classical counterpart. \\
There is no result asserting that the class of functionWe refer to (VAZIRANI) for a complete introduction to quantum complexity theory. 
%
%
%
\section{Reversible logic and the limit of computation}
Computers heat up, i.e. they dissipate energy, they are thus irreversible engines. It is not just a matter of imperfection in the construction of the components: they dissipate because they are based on irreversible logical components which throw information away. Landauer \cite{landauer61} that any erasure or overwriting of a bit generates an amount $k_B \ln 2$ of entropy. This logical irreversibility turns itself into heat dissipation at a reate of $k T \log 2$ units of heat per erased bit \cite{bennett82}.
%\emph{Se da un lato le leggi della fisica impongono una revisione dei concetti classici dell'informatica, dall'altro il rapido aumento del grado di miniaturizzazione delle componenti elettroniche degli attuali calcolatori, con i relativi problemi di dissipazione e rumore, hanno spinto molti ricercatori a porsi delle domande sui limiti dell'attuale tecnologia microelettronica. Le ricerche di Bremermann [5-a], Gupta [5-a], Likharev [5-a], Landauer [5-a] e Bennett [5-a] indagano i limiti della dissipazione di energia da parte delle porte logiche. In particolare Likharev mostra che l'utilizzo di dispositivi fisicamente reversibili diminuisce considerevolmente il limite minimo fondamentale di dissipazione, precedentemente fissato a aT (a indica la costante di Boltzmann).}
If on one side quantum mechanical effects seem to be exploitable both for the simulation  of quantum systems and to efficiently solve some hard problem, on the other side there is a ``passive'' reason to consider them: quantum effect are beginning to interfere in the functioning of electronic devices as they are made smaller and smaller. Considered the \emph{Moore's law}, which states that computer power will double for constant cost roughly once every two years, and the actual size of transistors (CARLO DE FALCO PER DATI SU MOSFET) it becomes clear that conventional approaches to the fabrication of computer technology will run up in a couple of decades.
%
\section{Principles of quantum computation}
Definizione di software e hardware di peres?
%
\section{Quantum algorithms and quantum walks}



==> chap_stochasticsim.tex <==
%\chapter{Stochastic simulation of a quantum walk} \label{chap:stochastic}
%\input{intro_stochasticsim.tex}
%\input{Brown}
%\input{Nelsquant}
%\input{Madelung}
%\input{Guerrapresc}
%\section{Simulation: some example}
%Here we show the Mathematica code and the simulations.

==> conclusionsandoutlook.tex <==

%


==> intro_quantumtiming.tex <==
%Introduzione Quantum timing and synchronization problems


\section{Introduction} \label{S:intro}
%
Computation is a physical process \cite{landauer82} and the intimate notion of computable function $f$ relies on the possibility of implementing a physical process transforming the input state $S_0$ in the desired output state $f(S_0)$ \cite{bennett82,toffoli82,vonNeumann76}.
\footnote{In \cite{toffoli82} Toffoli illustrated the equivalence between a physical experiment and a computing process by means of the following suggestive example:
\begin{quote}
Let us suppose that intelligent beings are observing us from a far away star. How could them understand whether we are carrying on a computation or a physical experiment? They could not understand it from what we are doing since there is no objective difference. The difference is in our intentions, in our knowledge, in our expectations.
\end{quote}
}.
The Church-Turing hypotheses \cite{church36,turing36,kleene43}
\begin{quotation}
Every function that would \emph{naturally be regarded as computable} can be computed by a universal Turing machine
\end{quotation}
itself makes an implicit physical assertion which was made explicit by Deutsch \cite{deutsch85}
\begin{quote}
Every finitely realizable physical system can be perfectly simulated by a universal model computing machine operating by finite means \footnote{This statement is also known as the \emph{Church-Turing-Deutsch} hypotheses.}.
\end{quote}
Quantum mechanics enters into play for two reasons: first, the law of physics are quantum mechanical; second modern physics relies heavily on computing devices to simulate physical systems but suffers of the exponential growth of the complexity of the simulation task with the dimension of the system to simulate. It was Feynman which suggested to use quantum mechanical devices to efficiently simulate quantum mechanical systems \cite{feyn82}.\\
Since the seminal works of Feynman the field of \emph{quantum computation} has known an enormous growth and nowadays it is a mature research field in between physics and computer science. We refer to \cite{nielsen} for an exhaustive introduction to the field of quantum computation and quantum information.\\[5pt]
%
In this work we present the quantum mechanical computer proposed by Feynman in 1985 (and, since then, almost forgotten). The main feature of the model is the presence of an built-in clocking mechanism managing for the ordered application of the computational primitives to the I/O register. Beside, it represents in some sense a generalization of  continuous time quantum walks  \cite{farhi97,childs02,farhi03}. Furthermore, since the clocking mechanism relies on a spin chain, any insight in the features of the computational model of Feynman can shed light onto the field of quantum communication via spin chains (cita bose e altri). \\[5pt]
Given a transformation $A$ to be applied to the input/output register, quantum computation starts from the decomposition of $A$ into the sequential application of simpler computational primitives, that is local transformations, $ U_n \cdot \ldots \cdot U_2 \cdot U_1$, which are unitary operators  acting on few qubits of the input output register at a time. The evolution of the input state into the output state is then seen as a discrete-stepwise process: at any time-step an operation is performed on the input/output register.\\
In general, in quantum mechanics, the outgoing state at time $t$ for a system with \emph{time-independent} Hamiltonian $H$ is $e^{-i H t} \ket{\psi_0}$ , where \ket{\psi_0} is the input state; in other words, the state of the system evolves under the action of the one continuous parameter unitary group generated by the Hamiltonian $H$. To try to find, for a given special time $\bar{t}$, the Hamiltonian which will produce $A = e^{-i H \bar{t}}$ when $A$ is a product of \emph{noncommuting} matrices $U_1,U_2,\ldots, U_n$, from some simple property of the matrices themselves, appears to be very difficult\footnote{For example, following the method proposed by Benioff \cite{benioff82} it is possible to define a time-independent Hamiltonian guiding the desired evolution from any input to any output state. The problem is that the explicit construction of such a Hamiltonian requires the prior knowledge of every step in the solution of every problem which the computer can solve}.\\
If one accepts a time-dependent Hamiltonians, it is fairly straightforward to write an Hamiltonian for the evolution of the input state into the output state via the indicated intermediate steps; keeping in mind the mechanism of a synchronous system, one can imagine an internal  clock turning the interactions on and off. This idealized clocking mechanism is though not satisfactory: a classical macroscopic clock would destroy the coherence of the quantum system so, to be consistent, the clock itself should be quantized; but as soon as we do it it becomes clear that this clock would be affected by whatever it interacts with \cite{peres80} and time steps would be blurred.\\
The problem of explicitly define a time-independent Hamiltonian driving the input state to the output state through the intermediate states determined by the \emph{ordered application} of the computational primitives was overcome by Feynman in 1985 \cite{feyn86}. This chapter is devoted to a description of the Feynman quantum computing device: we introduce the basic model and set the notation to be used throughout this thesis. For a detailed description of the model we refer to the original paper of Feynman and to \cite{defa04}.
%
\section{The basic model} \label{sec:themodel}
%
%The model we consider consists of two functionally distinct parts, the \emph{input/output register}  and the \emph{clock}  or \emph{cursor}, and evolves as an \emph{autonomous system} under the sole effect of its initial state not being an eigenstate of the Hamiltonian of the composite system.\\
%Let $\ket{R(1)}\in \Hr$ be the initial state of the input/output register.  Set
%\begin{equation}
%	d=dim(\Hr).
%\end{equation}
%Let \ves{U}{N-1} be the unitary operators representing the successive \emph{primitive} steps of the computation to be performed. Suppose, namely, that the goal of the computation is to transform the input state \ket{R(1)} into the output state $\ket{R(N)}= U_{N-1} \cdot \ldots U_2 \cdot U_1 \ket{R(1)}$   by visiting the successive intermediate states
%\begin{equation}
%	\ket{R(x)}= U_{x-1} \ket{R(x-1)},\ 1 < x < N.
%\end{equation}
%Following the approach of \cite{feyn86}, we model the clocking mechanism, which sequentially applies the transformations \ves{U}{N-1} to the register, with a quantum mechanical system, the \emph{cursor}.\\
%We call \Hc the $s$-dimensional ($s \geq N$) state space of this system and refer it to a selected orthonormal basis $\ket{C(1)},\ \ket{C(2)}$,\ldots,\ \ket{C(s)}. It will help the intuition, and will explain the notation used below, to think of an explicit implementation of the cursor by $s$ spin $1/2$ particles and to think of the state \ket{C(x)} as obtained by flipping ``up'' the spin in position $x$ with respect to the ``all down'' reference state.\\
%We suppose that the state of the overall system, the \emph{machine}, evolves in the Hilbert space $\Hm = \Hr \otimes \Hc$ under the action of a Hamiltonian of the form
%\begin{equation}\label{eq:hamiltoniana2}
%	H = -\frac{\lambda}{2} \sum_{x=1}^{s-1} U_x \otimes \ketbra{C(x+1)}{C(x)} + U_x^{-1} \otimes \ketbra{C(x)}{C(x+1)}.
%\end{equation}
%Notice that only \ves{U}{N-1} are assigned by the algorithm we are interested in; $U_N,\ldots, U_{s-1}$ are to be assigned as a part of the description of the clocking mechanism.\\[10pt]
%%
%
%
It has been shown by Feynman \cite{feyn86} that it is possible to implement the sequential application, in the desired order, of the sequence 
\[
 U_{s-1} \cdot \ldots \cdot U_2 \cdot U_1=A
\]
of unitary operators to an \emph{input/output register} by using \emph{s} additional degrees of freedom: the \emph{program counter sites}.\\
For the sake of definiteness, we will think of each program counter  site $j=1,2, \dots, s$ as occupied by a spin-1/2 system $ \underline{\tau}(j)=(\tau_1(j),\tau_2(j),\tau_3(j))$ living in an Hilbert space $\mathcal{H}$ isomorph to $\mathbb{C}^2$. We will refer to the collection of such spins, which act in effect as a quantum clocking mechanism, as to a \emph{program line}.\\ 
The \emph{input/output register} will be, similarly, implemented by a collection of a certain number $\mu$ \ of spin-1/2 systems $\underline{\sigma}(i)=(\sigma_1(i),\sigma_2(i),\sigma_3(i)):\mathcal{H} \rightarrow \mathcal{H},\; i=1,2, \dots,\mu $.\\
We remember that the generalized angular momentum operators $\underline{\tau}(\cdot)$ satisfy the canonical commutation relations (or CCR)\index{CCR}
\begin{eqnarray}\label{eq:ccr}
 \left[ \tau_1(x),\tau_2(y) \right ] & =  & \delta_{x,y}\frac{i}{2} \tau_3(x) \\
 \left[ \tau_3(x),\tau_1(y) \right ] & =  & \delta_{x,y}\frac{i}{2} \tau_2(x) \\
 \left[ \tau_2(x),\tau_3(y) \right ] & = & \delta_{x,y}\frac{i}{2} \tau_1(x).
\end{eqnarray}
Obviously the same conditions are satisfied by the $\underline{\sigma}$'s.\\ 
We reflect the functional separation of the subsystems, by calling  $\Hc = \mathcal{H}^{\otimes s}$ the Hilbert space in which the collection of the spin making up the cursor are defined; analogously we refer to the Hilbert space the register is located in as $\Hr = \mathcal{H}^{\otimes \mu}$. The overall system, \emph{register} + \emph{program line}  evolves in the space $\Hm =\Hr \otimes \Hc$ under the action of the Hamiltonian 
\begin{equation} \label{eq:hamfeynman}
H=-\frac{\lambda}{2}\Bigl ( \sum_{j=1}^{s-1}U_j \otimes\tau_+(j+1) \tau_-(j)  + U_j^{-1} \otimes\tau_+(j)\tau_-(j+1) \Bigr ).
\end{equation}
where
\begin{equation}
	\tau_{\pm}(j)=\frac{\tau_1(j)\pm i \tau_2(j)}{2}
\end{equation}
are respectively the \emph{raising} and \emph{lowering} (or \emph{excitation creation} and \emph{annihilation}) operators acting on the $j$-th spin of the cursor and $\lambda$ is a scalar coupling constant (for notational convenience, we will set $\lambda=1$ unless otherwise specified). For the sake of definiteness, for every spin of the system we will take the eigenstates of the $\tau_3$ (respectively $\sigma_3$) operator as the basis for the Hilbert space $\mathcal{H}$ of a single spin and indicate them by the eigenvalue $\pm$ of $\tau_3$ they belong to. This basis is conventionally referred to as \emph{computational basis}\index{computational basis} and the \emph{Pauli operators}\index{Pauli operators} $\tau_1,\ \tau_2,\ \tau_3$ have the usual matrix representation:
\begin{equation}
\tau_1 = \left (
\begin{array}{c c}
	0 & 1 \\
	1 & 0
\end{array}\right ) \;
\tau_2 = \left (
\begin{array}{c c}
	0 & -i \\
	i & 0
\end{array}\right )\;
\tau_3 = \left (
\begin{array}{c c}
	1 & 0 \\
	0 & -1
\end{array}\right )
\end{equation}
Throughout this work we will use \ket{\pm 1} to refer to the eigenstates \ket{\tau_3=\pm 1} respectively. When considering a collection on $n$ spins $\underline{\tau}(1),\underline{\tau}(2),\ldots,\underline{\tau}(n) \in \mathcal{H}^{\otimes n}$ we will refer it to the orthonormal basis made up of the eigenstates of $\bigotimes_{x=1}^n \tau_3(x)$, indicating them as
\begin{equation}
	\ket{\tau_3(1)=\pm 1,\tau_3(2)=\pm 1,\ldots,\tau_3(n) = \pm 1} = \ket{\underbrace{\pm 1,\pm 1,\ldots,\pm 1}_{n}}.
\end{equation}
The evolution of the computing device is given by the solution of the Cauchy problem:
%
\begin{equation}
\begin{cases}
i \frac{d}{dt} | \psi(t) \rangle = H | \psi(t) \rangle \\
\ket{\psi(0)}=\ket{\psi_0}
\label{eq 1}
\end{cases}
\end{equation}
%
where we have set $\hbar = 1$ for notational convenience.\\
We define the operator \emph{number of excitation}
%
\begin{eqnarray}
N_3 & : & \Hc \rightarrow \Hc \nonumber\\
N_3 & = & \sum_{j=1}^{s} \frac{1+\tau_3(j)}{2},
\end{eqnarray}
%
\begin{proposition} \label{th:number}
The number of spin up, or \emph{excitation} on the program line is a constant of motion that is
\begin{equation} \label{eq:n3}
[H,N_3]=0.
\end{equation}
\end{proposition}
\begin{proof}
Since $N_3$ acts only on the cursor, it we can trace out the register degrees of freedom. From the CCR defined above it follows:
\begin{eqnarray}
	[H,N_3]& = & [\sum_{x=1}^{s-1} \tau_+(x+1) \tau_-(x) + \tau_+(x) \tau_-(x+1),\sum_{y=1}^s \frac{1+\tau_3(x)}{2}] = \nonumber \\
	& = &   \frac{1}{2} \sum_{x=1}^{s-1} \sum_{y=1}^s \left( [ \tau_+(x+1) \tau_-(x), \tau_3(x)] + [ \tau_+(x) \tau_-(x+1), \tau_3(x)] \right ) = \nonumber \\
	& = &  \frac{1}{2}  \sum_{x=1}^{s-1} ([\tau_+(x+1) \tau_-(x), \tau_3(x)] + [\tau_+(x+1) \tau_-(x), \tau_3(x+1)] + \nonumber \\
	& + & [\tau_+(x) \tau_-(x+1), \tau_3(x)] + [\tau_+(x) \tau_-(x+1), \tau_3(x+1)]) =\nonumber \\
	& = & \frac{1}{2} \sum_{x=1}^{s-1} (\tau_+(x+1)[ \tau_-(x), \tau_3(x)] +\tau_-(x) [\tau_+(x+1) , \tau_3(x+1)] + \nonumber \\
	& + & \tau_-(x+1)[\tau_+(x) , \tau_3(x)] + \tau_+(x) [ \tau_-(x+1), \tau_3(x+1)]) =\nonumber \\
	& = & - \tau_+(x+1) \tau_-(x) + \tau_-(x)\tau_+(x+1) + \nonumber \\
	& + & \tau_-(x+1)\tau_+(x)-\tau_+(x)\tau_-(x+1) =0
  \end{eqnarray}
\end{proof}
A first consequence of proposition \ref{th:number} is that if the initial state of the cursor belongs to the $N_3=k$ subspace of \Hc, the state vector of the cursor lives in the subspace of  \Hc spanned by the $\left ( 
\begin{array}{c}
	s \\
	k
\end{array}
\right )$ basis vector
\begin{equation}
	\tau_+(j_1) \tau_+(j_2)\ldots \tau_+(j_k)\ket{0}, 1\leq j_1 < j_2 < \ldots < j_k \leq s
\end{equation}
where with \ket{0} we indicate the ``all-down'' state, that is the \ket{\tau_3(1)=\tau_3(2)=\ldots=\tau_3(s)=-1} state. The reduction of the dimensionality of the state vector, and thus the complexity of any simulation of the system, is therefore significantly reduced. In particular, we will usually restrict our considerations to initial conditions belonging to the $N_3=1$ subspace and refer the cursor subspace to the orthonormal basis 
\begin{equation} \label{eq:cj}
	\{ \ket{C(j)}=\tau_+(j)\ket{0},\;1\leq j\leq s \}.
\end{equation}
The initial state of the computing device will be of the form
%
\begin{equation}
\ket{\psi_1} =\ket{ R(1)} \rangle\otimes \ket{C(1)} .
\label{E:init}
\end{equation}
%
It helps the intuition to think of the initial state $\ket{R(1)}$ of the register as a simultaneous eigenstate of the components of the $\sigma$ spins in selected directions, encoding the initial word (or superposition of words) on which the machine is required to act.
%
The intuition of ``a single clocking excitation traveling along the program line'' emerging from the above considerations is made precise by introducing the observable \emph{position of the excitation}, or \emph{position of the cursor}:
%
\begin{equation} \label{eq:Q}
Q=\sum_{j=1}^{s}j \; \frac{1+\tau_3(j)}{2}.
\end{equation}
%
Let us have a look on the Hamiltonian \eqref{eq:hamfeynman} and on the  interaction of the program line with the register degrees of freedom it describes. At any particular time $t$, if we expand
\begin{equation}
	e^{-i H t} = 1 -i H t - H^2 t^2 / 2+ \ldots
\end{equation}
it becomes clear that the state of the system is a superposition of $H$ acting a numerable arbitrary number of times.\\
To illustrate the functioning of the clocking mechanism, we will consider only states of the form
\begin{equation}\label{eq:stdstate}
\ket{\psi_k}= \ket{R(k)} \otimes \ket{C(k)} ,\; 1 < k < s
\end{equation}
where by \ket{R(j)} we indicate the $(j-1)$-th logical successor of the initial state \ket{R(1)} of the register, that is
\begin{equation}
	\ket{R(j)} = U_{j-1} U_{j-2} \ldots U_2 U_1 \ket{R(1)},
\end{equation}
and the state of the cursor is a basis vector of the $N_3=1$ subspace of \Hc.\\
We begin with a look on the action of $H$ on a state of the form \eref{eq:stdstate}
\begin{eqnarray}
H \ket{\psi_k} & = & \sum_{x=1}^{s-1}U_x \otimes\tau_+(x+1)\tau_-(x)  \ket{\psi_k}+ U_{x}^{-1} \otimes \tau_+(x)\tau_-(x+1)  \ket{\psi_k} \nonumber \\
& = & U_k \ket{R(k)} \otimes\ket{C(k+1)}   +  U_k^{-1} \ket{R(k)}\otimes\ket{C(k-1)}  = \nonumber \\
& = & \ket{R(k+1)}\otimes\ket{C(k+1)}+   \ket{R(k-1)} \otimes \ket{C(k-1)} =  \nonumber \\
& =& \ket{\psi_{k+1}} + \ket{\psi_{k-1}}
\end{eqnarray}
We intentionally left out the case in which $H$ acts on the states \ket{\psi_1} and \ket{\psi_s}. In those cases, due to the boundary of the system, we have 
\begin{eqnarray}
	H \ket{\psi_1} & = & \ket{\psi_2} \\
	H \ket{\psi_s} & = & \ket{\psi_{s-1}}.
	\label{eq:boundary}
\end{eqnarray}
The coupling of the register with the cursor degrees of freedom seems to be of the following kind: if the excitation moves one step further, the logical state of the computation advances by one; if the excitation moves one step backward, the logical state regresses to the previous one. This property holds also when applying higher powers of the Hamiltonian operator to the system. For example, if we consider $H^2$  and expand it we get
\begin{eqnarray}
	H^2 & = & \sum_{x=1}^{s-1} \sum_{y=1}^{s-1}U_x U_y \otimes\tau_+(x+1)\tau_-(x)\tau_+(y+1)\tau_-(y)  + \nonumber \\
	& + &  U_x U_y^{-1}\otimes\tau_+(x+1)\tau_-(x)\tau_+(y)\tau_-(y+1) \nonumber \\
	& + &  U_x^{-1} U_y\otimes\tau_+(x)\tau_-(x+1)\tau_+(y+1)\tau_-(y) \nonumber \\
	& + & U_x^{-1} U_y^{-1}\otimes \tau_+(x)\tau_-(x+1)\tau_+(y)\tau_-(y+1). 
	\label{eq:h2expansion}
\end{eqnarray}
It is straightforward to see that, due to the CCR \eref{eq:ccr} and to the conservation law \eref{eq:n3} only some of the terms with $x=y$ and $x=y \pm 1$ survive. Thus, it is possible to simplify \eref{eq:h2expansion} getting
\begin{eqnarray}
	H^2 & = &\sum_{x=2}^{s-1} U_x U_{x-1}\otimes \tau_+(x+1)\tau_-(x)\tau_+(x)\tau_-(x-1)  + 	\nonumber \\
	& = & 1  \otimes\tau_+(x)\tau_-(x+1)\tau_+(x+1)\tau_-(x)+ \nonumber \\
	& = & 1  \otimes\tau_+(x+1)\tau_-(x)\tau_+(x)\tau_(x+1) + \nonumber \\
	& = &  U_{x-1}^{-1} U_{x-1}^{-1}\otimes\tau_+(x-1)\tau_-(x)\tau_+(x)\tau_-(x+1).
\end{eqnarray}
For example, if  $H$ acts twice on the state $ \ket{C(k)} \otimes \ket{R(k)} $, with $2 < k < s-2$ we get
\begin{eqnarray}
	H^2  \ket{R(k)} \otimes \ket{C(k)} & = & {U_{k+2} U_{k+1} \ket R(k)} \otimes \ket{C(k+2)}+ \nonumber \\
	 & + &  2   \ket{R(k)} \otimes \ket{C(k)}+\nonumber \\
	 & + &  U_{k-1}^{-1} U_{k}^{-1} \ket{ R(k)} \otimes \ket{C(k-2)}  .
\end{eqnarray}
Once more: if the position of the excitation is shifted by $j$-positions, $j \in \{0,2\}$ the logical state evolves or involves accordingly by $j$-steps. This property extends to every power of $H$; in fact, once defined the projection operator on the $k$-th logical state \ket{R(k)}
\begin{equation}
	P_k \ket{R(l)}= \delta_{k,l} \ket{R(k)}.
\end{equation}
that satisfies
\begin{equation}
	P_k = U_k P_{k-1}U_k^{-1}
\end{equation}
and the operator
\begin{equation} \label{eq:p}
	P=\sum_{k=1}^{s}  P_k \otimes \ketbra{C(k)}{C(k)} 
\end{equation}
the following holds
\begin{theorem}
\begin{equation}
[P,H]=0
\end{equation}
\end{theorem}
Before showing the proof, we observe that, given \eref{eq:stdstate} and proposition \ref{th:number} the Hamiltonian \eref{eq:hamfeynman} is equivalent to
\begin{eqnarray} \label{eq:hfeynman2}
H & = & \sum_{x=1}^{s-1}  U_x \otimes \ketbra{x+1}{x}+  U_x^{-1} \otimes \ketbra{x}{x+1}  =  \nonumber \\
	& = & \sum_{x=1}^{s-1}  U_x \ketbra{x+1}{x}  + U_x^{-1} \ketbra{x}{x+1}  
\end{eqnarray}
where \ket{x} is the eigenstate of the position operator $Q$ \eref{eq:Q} belonging to the eigenvalue $x$, and the tensor product symbol has been dropped to shorten the expressions. Equivalently \eref{eq:p} can be rewritten as
\begin{equation} \label{eq:p1}
	P=\sum_{k=1}^{s} P_k \ketbra{k}{k} .
\end{equation}
\begin{proof}
We compute explicitly $P\;H$ and $H\;P$.
\begin{eqnarray}
	P\; H & = & \sum_{k=1}^s P_k  \ketbra{k}{k} (\sum_{x=1}^{s-1} U_x \ketbra{x+1}{x}  + U_x^{-1}\ketbra{x}{x+1} ) = \nonumber \\
	& = &  \sum_{k=1}^s \sum_{x=1}^{s-1} P_k U_x\ket{k}\braket{k}{x+1}\bra{x}  + P_k U_x^{-1} \ket{k}\braket{k}{x}\bra{x+1}  \nonumber \\
	& = & \sum_{x=1}^{s-1} P_{x+1}U_x\ketbra{x+1}{x} + P_x U_x^{-1}\ketbra{x}{x+1}
\end{eqnarray}
\begin{eqnarray}
	H	\;P  & = &  (\sum_{x=1}^{s-1}U_x \ketbra{x+1}{x}  + U_x^{-1}\ketbra{x}{x+1} ) \sum_{k=1}^s P_k \ketbra{k}{k}   = \nonumber \\
	& = & \sum_{x=1}^{s-1} \sum_{k=1}^s  U_x P_k \ket{x+1}\braket{x}{k}\bra{k}   + U_x^{-1} \ket{x}\braket{x+1}{k}\bra{k}    \nonumber \\
	& = & \sum_{x=1}^{s-1} U_x P_{x}\ketbra{x+1}{x} +U_x^{-1} P_{x-1} \ketbra{x}{x+1} 
\end{eqnarray}
Thus
\begin{eqnarray}
PH-HP & = & (P_{x+1}U_x - U_x P_ x)\ketbra{x+1}{x}+ (P_x U_x^{-1} - U_x^{-1} P_{x+1})\ketbra{x}{x+1} = \nonumber \\
 & = & (U_x P_{x}U_x^{-1} U_x - U_x P_ x)\ketbra{x+1}{x}  +  \nonumber \\ 
 & + & (P_x U_x^{-1} - U_x^{-1} U_x P_{x}U_x^{-1})\ketbra{x}{x+1} = 0
\end{eqnarray}
\end{proof}
The space spanned by the initial state and the logical successor is thus a constant of motion. The set $\left \{ \ket{\psi_k}, 1 \leq k \leq s \right \}$  forms a complete orthogonal basis for the $s$-dimensional subspace of \Hm effectively visited during the computation. It is worth mentioning here that the set of logical successor of the initial state, or \emph{Peres' basis} \index{Peres' basis}, can be algorithmically constructed; in fact, if we split the Hamiltonian  \eref{eq:hfeynman2} into
\begin{eqnarray}
H_{forward} & = & \sum_{x=1}^{s-1}  U_x \ketbra{x+1}{x} \\
H_{backward} & = & \sum_{x=1}^{s-1}  U_x^{-1} \ketbra{x}{x+1};
\end{eqnarray}
the set of logical successors of the initial state \ket{\psi_1} corresponds to then the set
\begin{equation} \label{eq:costruzioneperes}
	\{ \ket{\psi_k} = H_{forward}^{k-1} \ket{\psi_1},\; 1 \leq k \leq s \}
\end{equation}
The Hamiltonian  \eref{eq:hfeynman2} can be rewritten in using the Peres basis as
\begin{equation}
	H = \sum_{k=1}^{s-1} \ketbra{\psi_{k+1}}{\psi_k} + \ketbra{\psi_{k}}{\psi_{k+1}}
\end{equation}
or as a $s \times s$ bi-diagonal matrix
\begin{equation} \label{eq:hmatrix}
	H = \left (
\begin{array}[pos]{c c c c c c}
0 & 1 & 0 & \ldots & 0 & 0\\
1 & 0 & 1 & \ldots & 0 & 0\\
0 & 1 & 0 & \ldots & 0 & 0\\
\ldots & \ldots & \ldots & \ldots & \ldots & \ldots\\
0 & 0 & 0 & \ldots &  0& 1\\
0 & 0 & 0 & \ldots & 1 & 0
\end{array} \right ).
\end{equation}
which is the finite difference approximation of the Laplace operator. The evolution of the system is thus  of the form
%
\begin{equation} \label{eq:psit}
| \psi(t) \rangle= \sum_{k=1}^s c(t,k,s) \;  \ket{\psi_k}  = \sum_{k=1}^s c(t,k,s) \;  \ket{R(k)} \otimes \ket{C(k)}
\end{equation}
$c(t,k,s)$ being numerical functions of the time $t$, of the label of the logical successor $k$ and parametric with respect to the length of the program line. For the sake of simplicity we postpone the discussion of the $c(t,k;s)$ coefficient to chapter \ref{chap:quantumtiming}.\\
%
From \eref{eq:psit} it becomes clear how the clocking mechanism works: if a measurement is performed and the cursor is found at position $N$, then the register is in the $N-1$ logical successor of the initial state \ket{R(1)}. In particular, if the cursor is found in the last site, the $s$-th in our notation, the logical state of the register corresponds to the desired output state, that is $A \ket{R(1)}$. In Feynman's words (adapted to our notations), (\ref{eq:psit}) says that, starting from the initial condition (\ref{E:init}), ``\underline{If} at some later time the final site $s$ is found to be in the  $| \tau_3(s)=+1 \rangle$  state (and therefore all the others in $| \tau_3(j)=-1 \rangle$ ), then the register state has been multiplied by $U_{s-1}\cdot \dots \cdot U_2 \cdot U_1$  as desired''.


==> intro_stochasticsim.tex <==
%\subsection{Introduction.} \label{sec:intro}
During the 50ies, Bohm and Vigier introduced a model of causal interpretation of quantum mechanics in which quantum fluctuations were seen as fluctuations of a Madelung fluid \cite{bohm53}\cite{bohm54}. The main idea was that a particle, e.g. an electron, follows a continuous causally defined trajectory with a well-defined position $\xi(t)$, accompanied by a physical real wave $\psi(x,t)$. In order to obtain all the results of the usual interpretation of quantum mechanics, the following assumptions had to be made:
\begin{enumerate}
\def\theenumi{\roman{enumi}}
\item $\psi(x,t)$ satisfies the Schr\"odinger equation;
\item $d\xi /dt = \nabla S /m$, where $\psi(x,t)= R \exp(i S /\hbar)$ (de Broglie form of the wave function);
\item the probability distribution in an ensemble of electrons having the same wave function is $P=|\psi|^2$.
\end{enumerate}
Given an ensemble of trajectories, the derivative of the density gives a \emph{quantum potential} which, in turn, determines the mean evolution of the system, in a similar way pressure in a classical fluid does. The key concept of the theory of Bohm and Vigier is
\begin{quotation}
Since the Madelung fluid is being assumed to be some kind of physically real fluid, it is therefore quite natural to suppose that it too undergoes more or less random fluctuations in its motion. Such random fluctuations are evidently consistent within the framework of the causal interpretation of quantum theory. Thus, there are always random perturbations of any quantum mechanical system which arise outside that system.\cite{bohm54}
\end{quotation}
%Stochastic mechanics is the description of quantum phenomena in classical probabilistic terms. 
In 1967 Nelson \cite{nelson67} gave a stochastic interpretation of quantum mechanics starting from the hypothesis that the evolution of a microscopic particle, e.g. an electron, is a Markov process.
\begin{quotation}
\ldots perhaps quantum fluctuation are real, and have physical causes. 
No physical system of finite degrees of freedom is truly isolated; it is always an interaction with a background field. (\ldots) The \emph{background field hypothesis} is that the interaction with the background field causes the system to undergo a diffusion process.\cite{nelson85}
\end{quotation}
The theory of Nelson, which is known as Nelson stochastic mechanics, can therefore be seen as a specialization of the theory of Bohm, since it identifies in the Brownian motion of the interacting background field the origin of the perturbations of the quantum system (whereas Bohm left the identification of such an origin as an open problem).\\[5pt]
In this work we are concerned with the stochastic quantization of a discrete quantum system. In particular, we are going to simulate sample paths of an excitation traveling on a linear chain of spin $1/2$ particles. We use the prescription of Guerra \cite{guerra84} to obtain the transition probabilities of the Markov process associated to the discrete quantum system.

==> introfqc.tex <==
We present Feynman' model of a quantum computer stressing the role of the clocking mechanism. We introduce the notion of logical successor of a given state and the related notion of Peres' constants of motion. We furthermore set the notation used throughout this work.
%\section{Introduction} \label{S:intro}
%
%Computation is a physical process \cite{landauer82} and the notion of computable function, say $f$, relies on the possibility of implementing a physical process transforming the input state $S_0$ in the desired output state $f(S_0)$ \cite{bennett82,toffoli82,vonNeumann76}.
%\footnote{In \cite{toffoli82} Toffoli illustrated the equivalence between a physical experiment and a computing process by means of the following suggestive example:
%\begin{quote}
%Let us suppose that intelligent beings are observing us from a far away star. How could they understand whether we are carrying on a computation or a physical experiment? They could not understand it from what we are doing since there is no objective difference. The difference is in our intentions, in our knowledge, in our expectations.
%\end{quote}
%}.
%The Church-Turing hypotheses \cite{church36,turing36,kleene43}
%\begin{quote}
%Every function that would \emph{naturally be regarded as computable} can be computed by a universal Turing machine
%\end{quote}
%makes itself an implicit physical assertion which was made explicit by Deutsch \cite{deutsch85}
%\begin{quote}
%Every finitely realizable physical system can be perfectly simulated by a universal model computing machine operating by finite means \footnote{This statement is also known as the \emph{Church-Turing-Deutsch} hypotheses.}.
%\end{quote}
%CAMBIARE:Quantum mechanics enters into play for two reasons: first, the law of physics are quantum mechanical; second modern physics relies heavily on computing devices to simulate physical systems but suffers the exponential growth of the complexity of the simulation task with the dimension of the system to simulate. It was Feynman who suggested to use quantum mechanical devices to efficiently simulate quantum mechanical systems \cite{feyn82}.\\
%Since the seminal works of Feynman the field of \emph{quantum computation} has known an enormous growth and nowadays it is a mature research field in between physics and computer science. We refer to \cite{nielsen} for an exhaustive introduction to the field of quantum computation and quantum information.\\[5pt]
%%
%In this work we present the quantum mechanical computer proposed by Feynman in 1985 (and, since then, widely cited but never used). The main feature of the model is the presence of a built-in clocking mechanism managing for the ordered application of the computational primitives to the input/output register.\\
%Given a transformation $A$ to be applied to the input/output register, quantum computation starts from the decomposition of $A$ into the sequential application of simpler computational primitives, $ U_n \cdot \ldots \cdot U_2 \cdot U_1$, which are unitary operators  acting on few qubits of the input output register at a time. The evolution of the input state into the output state is then seen as a discrete-stepwise process: at any time-step an operation is performed on the input/output register.\\
%In general, in quantum mechanics, the outgoing state at time $t$ for a system with \emph{time-independent} Hamiltonian $H$ is $e^{-i H t} \ket{\psi_0}$ , where \ket{\psi_0} is the input state; in other words, the state of the system evolves under the action of the continuous parameter unitary group generated by the Hamiltonian $H$. To try to find, for a given special time $\bar{t}$, the Hamiltonian which will produce $A = e^{-i H \bar{t}}$ when $A$ is a product of \emph{noncommuting} matrices $U_1,U_2,\ldots, U_n$, from some simple property of the matrices themselves, appears to be very difficult\footnote{For example, following the method proposed by Benioff \cite{benioff82} it is possible to define a time-independent Hamiltonian guiding the desired evolution from any input to any output state. The problem is that the explicit construction of such a Hamiltonian requires the prior knowledge of every step in the solution of every problem which the computer can solve}.\\
%If one accepts time-dependent Hamiltonians, it is fairly straightforward to write a Hamiltonian for the evolution of the input state into the output state via the indicated intermediate steps; keeping in mind the mechanism of a synchronous system, one can imagine an internal  clock turning the interactions on and off. This idealized clocking mechanism is however not satisfactory: a classical macroscopic clock would destroy the coherence of the quantum system so, to be consistent, the clock itself should be quantized; but as soon as we do it it becomes clear that this clock would be affected by whatever it interacts with \cite{peres80} and time steps would be blurred.\\
%The problem of explicitly define a time-independent Hamiltonian driving the input state to the output state through the intermediate states determined by the \emph{ordered application} of the computational primitives was overcome by Feynman in 1985 \cite{feyn86}.\\
%It has been observed by Margolus \cite{margolus90} that Feynman, in his model of a quantum computer,`managed to arrange for all the quantum uncertainty[...] to be concentrated in the time taken for the computation to be completed, rather than in the correctness of the answer'.\\
%Recent work by Levitin and Margolus \cite{levitin98} relates the maximum rate of information processing by a quantum computer to the available, \emph{conserved}, energy. It is therefore of some theoretical interest to revisit a model, such as Feynman's, based on a closed system, evolving according to a time-independent and, therefore, conserved Hamiltonian.\\
%The doubt has been raised by Alicki \cite{alicki00} that `the idea that the physical time[...] of computation is proporional to the complexity [...] is only true fo the existing digital computers which are ensembles of controlled bistable elements which [...] can literally mimic logical operations'.\\
%Feynman's model provides an ideal context for the study of this issue: timing is modeled by a cursor, which jumps along a sequence of sites, indicating that the corresponding discrete operations should be applied. \\[10pt]
%This chapter is devoted to a description of the Feynman quantum computing device: we introduce the basic model and set the notation to be used throughout this thesis. For a detailed description of the model we refer to the original paper of Feynman and to \cite{defa04}.
%%


==> qtsp_conclusions.tex <==
% Da Quantum timing and synchronization problems

\section{Conclusions and Outlook}\label{S:conclusions}
Feynman's time honoured model of a quantum computer and its modern streamlined version, the continuous-time quantum walk\cite{childs02} paradigm (in which the quantum motion of the {\it cursor} on a graph \underline{is} the computation, irrespective of any action on the register), provide a fascinating physical context in which to think of ``time'' under a quantum perspective and are rich sources of open problems.\\
Inequality (\ref{E:probnotelo}) is, for istance, a simple consequence of the spreading of the wave packet in the inertial motion (\ref{gramsscoeff}) of the cursor on a finite lattice. Is inequality (\ref{E:probnotelo}) strictly dependent on the model adopted here or is it a hint of a model independent ``probability vs. computational complexity'' uncertainty relation?\\
Inequality (\ref{E:upperbound}) and the related discussion of Sec.~\ref{S:pipulse} set bounds on the minimun amount of additional space needed in order to have a preassigned probability of storing the result of the complete calculation. Similarly, the preparation of a given input requires time and space in order to perform the required ``Stern-Gerlach'' preparation. Is it realistic to neglect this costs as it is done in the conventional performance analysis of performance of quantum algorithms?\\[4pt]
As a concluding remark, we wish to point out a case, Grover's algorithm\cite{grover96}, in which the nature, classical or quantum, of the clocking agent that successively applies the required primitives does make a difference.\\
Grover's algorithm poses the problem of estimating the parameters $\mathbf{a}=(a_1,\dots,a_{\mu} )\in \{-1,+1\}^{\mu}$ appearing in the transformation $\mathbf{A}=1-2 P_\mathbf{a}$ that an \emph{oracle} is able to apply to the register. Here we have indicated by $P_\mathbf{a}$ the projector on the state $|\sigma_3(i)=a_i,\; i=1,\dots,\mu \rangle \equiv | \mathbf{a}_3 \rangle$.\\
The estimation procedure of {\bf a} starts from $|register_0 \rangle=$ \mbox{$| \sigma_1(i)=+1,\; i=1,\dots,\mu \rangle$} $\equiv | \mathbf{1}_1 \rangle$ and proceeds by alternating the action of {\bf A} with the action of $\mathbf{B}=1-2 |\mathbf{1}_1 \rangle \langle \mathbf{1}_1 |$.\\
It can be shown\cite{boyer98} that:
%
\begin{equation}
\label{E:amplsol}
| \langle \mathbf{a}_3|(\mathbf{B} \cdot \mathbf{A})^n | \mathbf{1}_1 \rangle |^2 =\sin^2((2n+1) \vartheta),\mbox{ with }\vartheta=\arcsin(2^{-\mu / 2}).
\end{equation}
%
The sharp maximum of (\ref{E:amplsol}) at $n=n_{optimal} \approx \frac{\pi}{4} 2^{\mu /2}$ keeps reappearing periodically if the computation proceeds indefinitely after $n_{optimal}$ steps.\\
In \cite{farhi97} and \cite{farhi03}, the oscillatory nature of the overlap (\ref{E:amplsol}) between the target state $|\mathbf{a}_3 \rangle$ and the current state $(\mathbf{B} \cdot \mathbf{A})^n |\mathbf{1}_1 \rangle$ has been nicely explained in terms of the spectral gap of an analogue Hamiltonian of the form $- \gamma |\mathbf{a}_3 \rangle \langle \mathbf{a}_3| - |\mathbf{1}_1 \rangle \langle \mathbf{1}_1| $ acting on the \emph{register} viewed as an isolated system.\\[4pt]
In the context of the model considered in the previous sections, Grover's algorithm corresponds to the execution of a \emph{program line} of the form (\ref{E:firsth}) with $A_j = \mathbf{A}$ for odd $j$, $A_j = \mathbf{B}$ for even $j$.\\
Starting form the initial condition $ | \psi(0)\rangle = | \mathbf{1}_1 \rangle \otimes | Q=1 \rangle $, and taking, for the sake of definiteness, an odd value of $s$, $s=2g+1$, it is easy to check that the overlap probability is, in this case, given by
%
\begin{eqnarray}
\label{E:damping}
\langle\psi(t) | P_{\mathbf{a}} | \psi(t) \rangle & = & \sum_{n=0}^{g} \sin^2((2n+1) \vartheta)\bigl(|c(t,2n+1;s)|^2+ |c(t,2n+2;s)|^2 \bigr)= \nonumber \\ 
& = & \sum_{x=1}^{s} |c(t,x;s)|^2 \sin^2(\vartheta \; x_{odd}),
\end{eqnarray}
%
where $x_{odd}$ is the largest odd number not larger than $x$.\\
Direct inspection of (\ref{E:damping}) shows that (\ref{E:amplsol}) gives the {\it \underline{conditional}} probability of finding the register in the target state, \emph{given} that the cursor is in the state $| Q= 2n+1 \rangle $; in loose terms: the oscillatory behaviour (\ref{E:amplsol}) describes the overlap probability as a function of the ``machine time'', namely the position $Q$ of the clocking excitation.\\
%
\begin{figure}[!h]
\hspace{2cm}
\begin{picture}(180,130)(0,0)
\centering
\includegraphics[width=8cm]{./Figure/damping.eps}
\end{picture}
\begin{picture}(10,130)
\put(50,11){t}
\end{picture}
\caption{$ \mu=5$; $s=2^{\mu + 1}+1=65$.}
\label{F:damping}
\end{figure}
%
The right hand side of (\ref{E:damping}) gives, instead, the overlap probability as a function of the ``Galileian time'' $t$, the independent variable in (\ref{eq 1}).\\
Figure \ref{F:damping} shows the behaviour of $\langle\psi(t) | P_{\mathbf{a}} | \psi(t) \rangle $ as a function of $t$: the coupling of the \emph{register} with the \underline{many} clocking degrees of freedom has a damping effect on the oscillation of the state of the register.\\
In the example just discussed we have used, in fact, a number of clocking degrees of freedom growing exponentially with $\mu$. It is shown in \cite{defa03} and \cite{tama03} that the above pseudo-dissipative effect can still be observed if, by a careful use of \emph{quantum subroutines}, the number of program line sites is reduced to a polynomial in $\mu$. 

==> subroutines.tex <==
\section{Iteration of quantum subroutines}
Iteratore 

==> themodel.tex <==
\section{The model}
%
For instance, Reference \cite{apolloni02} presents the case in which $U_N,\ldots, U_{s-1}=I_r$, the identity in \Hr,  and shows the role of the cursor sites $N,\ldots,s$  as a storage mechanism of the output \ket{R(N)}.\\
An alternative point of view was taken in some of the numerical examples of \cite{defa04}, motivated by Grover's algorithm: one may suppose all of the $U_x$ to coincide, in such a context, with Grover's $estimation \cdot oracle$ step $G$, and study the effect of applying $G$ more than the optimal number $N-1$ of times.\\
This point of view will be taken also in some numerical examples of this paper, where we focus our attention on a Hamiltonian of the form:
\begin{equation} \label{eq:hamiltoniana3}
	H = -\frac{\lambda}{2} \sum_{x=1}^{s-1} U_x \otimes \tau_+(x+1) \tau_-(x) + U_x^{-1} \otimes \tau_+(x)\tau_-(x+1).
\end{equation}
Most of our numerical examples will refer in fact to the following particular instance (Toy model):
\begin{equation} \label{eq:hamiltoniana4}
		H_T = -\frac{\lambda}{2} \sum_{x=1}^{s-1} e^{-i\frac{\alpha}{2} \sigma_2} \tau_+(x+1) \tau_-(x) + e^{i\frac{\alpha}{2} \sigma_2}\tau_+(x)\tau_-(x+1).
\end{equation}
Here $\underline{\sigma}=(\sigma_1, \sigma_2, \sigma_3)$ is the single register spin $1/2$ that we are going to consider in our model; the cursor subsystem is implemented as a collection of spin $1/2$ systems $\underline{\tau}(j)=(\tau_1(j),\tau_2(j),\tau_3(j))$ , $j \in {1,\ldots,s}$, and $\tau_{\pm}(j)= (\tau_1(j)\pm i \tau_2(j))/2$.\\
The Hamiltonian \eref{eq:hamiltoniana2} can, of course, be considered as the restriction of \eref{eq:hamiltoniana3} to the eigenspace belonging to the eigenvalue $1$ of 
\begin{equation}
	N_3=\sum_{x=1}^s \frac{1+\tau_3(x)}{2},
\end{equation}
provided we identify $\ket{C(x)}$ with the simultaneous eigenstate of $\ve{\tau_3}{s}$ in which only  $\tau_3(x)$ has eigenvalue $+1$.    
